Kick Back & Relax: Learning to Reconstruct the World by Watching SlowTV

Self-supervised monocular depth estimation (SS-MDE) has the potential to scale to vast quantities of data. Unfortunately, existing approaches limit themselves to the automotive domain, resulting in models incapable of generalizing to complex environments such as natural or indoor settings. To address this, we propose a large-scale SlowTV dataset curated from YouTube, containing an order of magnitude more data than existing automotive datasets. SlowTV contains 1.7M images from a rich diversity of environments, such as worldwide seasonal hiking, scenic driving and scuba diving. Using this dataset, we train an SS-MDE model that provides zero-shot generalization to a large collection of indoor/outdoor datasets. The resulting model outperforms all existing SSL approaches and closes the gap on supervised SoTA, despite using a more efficient architecture. We additionally introduce a collection of best-practices to further maximize performance and zero-shot generalization. This includes 1) aspect ratio augmentation, 2) camera intrinsic estimation, 3) support frame randomization and 4) flexible motion estimation. Code is available at https://github.com/jspenmar/slowtv_monodepth.

==> Figures/preds.tex <==
% Zero-shot depth estimation.

\def\w{0.105}
\scriptsize

\def\datas{
    img/Image
    ,depth/GT
}

\def\selfsup{
    % ,garg/Garg~\cite{Garg2016}
    % ,monodepth2_MS/Monodepth2~\cite{Godard2019}
    hrdepth_MS/HR-Depth
    ,base/Ours
}

\def\sup{
    MiDaS/MiDaS
    % ,DPT_Large/DPT-ViT~\cite{Ranftl2021}
    ,DPT_BEiT_L_512/DPT-BEiT
    ,newcrfs/NeWCRFs
}


\def\nums{
    viz_base/kitti_eigen_benchmark_0072%
    ,viz_zero_out/syns_test_0374%
    ,viz_zero_out/sintel_0411%
    ,viz_base/mc_0938%
    ,viz_zero_out/ddad_0737%
    ,viz_zero_out/diode_outdoor_0030%
    ,viz_zero_in/diode_indoors_0139%
    ,viz_zero_in/nyud_0247%
    ,viz_zero_in/tum_0246%
}

\def\ds{
    Kitti
    ,SYNS
    ,Sintel
    ,Mannequin
    ,DDAD
    ,DIODE
    ,DIODE
    ,NYUD-v2
    ,TUM
}

\def\divider{\textcolor{black}{\hdashrule[1mm][x]{\linewidth}{\heavyrulewidth}{2pt}}}

\noindent
\rotatebox{90}{\color{white}{\textbf{\scriptsize Tmp}}}
\foreach \d in \ds{\makebox[\w\linewidth][c]{\textbf{\scriptsize\d}}\hfill}

\foreach \method/\label in \datas{%
    \rotatebox{90}{\textbf{\scriptsize \label}}
    \foreach \num in \nums{% 
        \includegraphics[width=\w\linewidth]{\num_\method}\hfill%
    } \\
}

\divider

\foreach \method/\label in \selfsup{%
    \rotatebox{90}{\textbf{\scriptsize \label}}
    \foreach \num in \nums{% 
        \includegraphics[width=\w\linewidth]{\num_\method}\hfill%
    } \\
}

\divider

\foreach \method/\label in \sup{%
    \rotatebox{90}{\textbf{\scriptsize \label}}
    \foreach \num in \nums{% 
        \includegraphics[width=\w\linewidth]{\num_\method}\hfill%
    } \\
}

\mycaption{Zero-shot \acl{ssmde}}{%
The proposed model adapts to a wide range of datasets and environments.
It greatly outperforms the updated self-supervised baselines from~\cite{Spencer2022,Lyu2021} and performs on-par with \ac{sota} supervised baselines~\cite{Ranftl2020,Ranftl2021,Yuan2021}, whilst being more efficient.
\emph{Middle=Self-Supervised -- Bottom=Supervised.}
}


==> Figures/slowtv.tex <==
% SlowTV sample images.

\def\w{0.166}

\foreach \img in {natural,driving,underwater}{%
    \foreach \num in {00, 01}{%
        \includegraphics[width=\w\linewidth]{slowtv/\num_\img}%
    }%
}%
\\[-0.3ex]
\foreach \img in {natural,driving,underwater}{%
    \foreach \num in {02, 03}{%
        \includegraphics[width=\w\linewidth]{slowtv/\num_\img}%
    }%
}%


\mycaption{\acl{stv}}{%
Sample images from the proposed dataset, featuring diverse scenes for hiking, driving and scuba diving. 
The dataset consists of 40 videos curated from YouTube, totalling to 1.7M frames. 
Diversifying the training data allows our \acl{ssmde} models to generalize to unseen datasets.
}

\vspace*{-0.4cm}


==> Figures/supp_preds_fail.tex <==
% Zero-shot depth estimation failure cases.

\def\w{0.103}

\def\datas{
    img/Image
    ,depth/GT
}

\def\selfsup{
    % ,garg/Garg~\cite{Garg2016}
    % ,monodepth2_MS/Monodepth2~\cite{Godard2019}
    hrdepth_MS/HR-Depth
    ,base/Ours
}

\def\sup{
    MiDaS/MiDaS
    % ,DPT_Large/DPT-ViT~\cite{Ranftl2021}
    ,DPT_BEiT_L_512/DPT-BEiT
    ,newcrfs/NeWCRFs
}

\def\nums{
    viz_base/kitti_eigen_benchmark_0234%
    ,viz_zero_out/syns_test_0026%
    ,viz_zero_out/sintel_0086%
    ,viz_base/mc_0513%
    ,viz_zero_out/ddad_0521%
    ,viz_zero_out/diode_outdoor_0336%
    ,viz_zero_in/diode_indoors_0110%
    ,viz_zero_in/nyud_0055%
    ,viz_zero_in/tum_0668%
}

\def\ds{
    Kitti
    ,SYNS
    ,Sintel
    ,Mannequin
    ,DDAD
    ,Diode
    ,Diode
    ,NYUD
    ,TUM
}

\def\divider{\textcolor{black}{\hdashrule[2mm][x]{\linewidth}{\heavyrulewidth}{2pt}}}


\noindent
\rotatebox{90}{\color{white}{\textbf{\scriptsize Tmp}}}
\foreach \d in \ds{\makebox[\w\linewidth][c]{\textbf{\scriptsize\d}}\hfill}

\foreach \method/\label in \datas{%
    \rotatebox{90}{\textbf{\scriptsize \label}}
    \foreach \num in \nums{% 
        \includegraphics[width=\w\linewidth]{\num_\method}\hfill%
    } \\
}

\divider

\foreach \method/\label in \selfsup{%
    \rotatebox{90}{\textbf{\scriptsize \label}}
    \foreach \num in \nums{% 
        \includegraphics[width=\w\linewidth]{\num_\method}\hfill%
    } \\
}

\divider

\foreach \method/\label in \sup{%
    \rotatebox{90}{\textbf{\scriptsize \label}}
    \foreach \num in \nums{% 
        \includegraphics[width=\w\linewidth]{\num_\method}\hfill%
    } \\
}

\mycaption{Failure Cases}{%
The proposed model occasionally produces holes of infinite depth or texture-copy artefacts. 
However, complex regions such as foliage or boundaries tend to be oversmoothed by all approaches. 
Finally, the upright prior in training data makes the model less robust to strong rotations. 
\emph{Middle=Self-Supervised -- Bottom=Supervised.}
}


==> Figures/supp_preds_motion.tex <==
% Zero-shot depth estimation failure cases.

\def\w{0.2}
% \def\w{0.24}

\def\datas{
    img/Image
    ,depth/GT
}

\def\models{
    full_no_md2_042/Baseline
    ,full_md2_042/Monodepth2
}

\def\nums{
    viz_motion/kitti_eigen_benchmark_0408%
    ,viz_motion/ddad_0973%
    ,viz_motion/sintel_0570%
    ,viz_motion/tum_1064%
}


\foreach \method/\label in \datas{%
    \rotatebox{90}{\textbf{\scriptsize \label}}
    \foreach \num in \nums{% 
        \includegraphics[width=\w\linewidth]{\num_\method}\hfill%
    } \\
}

\foreach \method/\label in \models{%
    \rotatebox{90}{\textbf{\scriptsize \label}}
    \foreach \num in \nums{% 
        \includegraphics[width=\w\linewidth]{\num_\method}\hfill%
    } \\
}

\mycaption{Monodepth2 Losses}{%
Monodepth2~\cite{Godard2019} reduces the presence of holes of infinite depth and dynamic object artefacts. 
The sharpness of object boundaries are also improved due to the refined correspondences from the minimum reconstruction loss. 
}


==> Figures/supp_slowtv.tex <==
% Supplementary SlowTV images (one per video). 

\newcommand{\numrows}{8}
\newcommand{\numcols}{5}
\def\w{.18}

\newcounter{i}
\newcounter{j}
\newcounter{ij}

% Zero-padding for sequence number
\renewcommand{\theij}{%
  \ifnum\value{ij}<10 0\fi
  \ifnum\value{ij}<100 000\fi
  \the\value{ij}%
}

\forloop{i}{0}{\value{i}<\numrows}{%
    \forloop{j}{0}{\value{j}<\numcols}{%
        \setcounter{ij}{\value{i}*\numcols + \value{j}}%
        \includegraphics[width=\w\linewidth]{slowtv_all/\theij}%
    } \\[-0.3ex]

}
\mycaption{\acl{stv} Dataset}{%
We show one frame per video from the proposed \acl{stv}. 
The dataset contains a diverse set of environments in a range of environmental conditions. 
The final dataset has a total of 1.7M images, with 1.15M natural, 400k driving and 180k underwater.
}


==> Tables/reb_dynamic.tex <==

\def\mc{\multicolumn}
\addtolength{\tabcolsep}{0.2em}
\footnotesize

\mycaption{Dynamic Object Results}{%
The losses from Monodepth2 improve performance in datasets with dynamic objects, despite not explicitly modelling their motion.
This ablation was conducted using ConvNeXt-Tiny and a small subset of all datasets.
}

\begin{tabular}{@{}llllllllll@{}}
\toprule
                 & \mc{2}{c}{\textbf{\acs{keb}}} & \mc{2}{c}{\textbf{\acs{ddad}}} & \mc{2}{c}{\textbf{\acs{sintel}}} \\ 
                              \cmidrule(lr){2-3}               \cmidrule(lr){4-5}                 \cmidrule(lr){6-7}
                 &     Rel\down & F\up &      Rel\down &          F\up &      Rel\down & F\up \\ 
\midrule
Baseline         & \nbest{9.00} & \nbest{53.50} & \nbest{23.57} & \nbest{11.13} & \nbest{35.33} & \nbest{38.15} \\ 
MinRec+Automask  &  \best{6.50} &  \best{55.62} &  \best{18.49} &  \best{11.64} &  \best{34.97} &  \best{38.83} \\ 
\bottomrule
\end{tabular}


==> Tables/reb_kitti.tex <==

\def\mc{\multicolumn}
\addtolength{\tabcolsep}{0.2em}
\small

\mycaption{\acl{kez} Results}{%
Learning \acs{Cam} gives comparable performance even when training only on Kitti.
}


\begin{tabular}{@{}llll@{}}
\toprule
                &     Rel\down &          F\up & \acs{d25}\up \\ 
\midrule
Baseline        & \nbest{5.69} &  \best{60.88} &     \nbest{95.89} \\ 
Learn \acs{Cam} &  \best{5.68} & \nbest{60.81} &      \best{95.90} \\ 
\bottomrule
\end{tabular}


==> Tables/res.tex <==
% Results on all datasets.

\scriptsize
\addtolength{\tabcolsep}{0.05em}
\def\mc{\multicolumn}

\mycaption{Results}{%
\textit{Outdoor} and \textit{Indoor} represent zero-shot evaluations. 
We outperform all \acl{ssmde} baselines~\cite{Spencer2022} (top block).
In many cases, our model performs on par with supervised \ac{sota} (bottom block), without requiring ground-truth depth annotations for training. 
}

\begin{tabular}{@{}llllllllllllllllllllll@{}}
\toprule
                             &       &&& \mc{4}{c}{\bf{In-Distribution}}                                         & \mc{8}{c}{\bf{Outdoor}}                                                                                                       & \mc{6}{c}{\bf{Indoor}}                                                                            \\
                                       \cmidrule(lr){5-8}                                                        \cmidrule(lr){9-16}                                                                                                             \cmidrule(lr){17-22}
                             &       & \mc{2}{c}{\textbf{Multi-task}} & \mc{2}{c}{\bf\acs{keb}}            & \mc{2}{c}{\bf\acs{mc}}             & \mc{2}{c}{\bf\acs{ddad}}      & \mc{2}{c}{\bf\acs{dio}}       & \mc{2}{c}{\bf\acs{sintel}}    & \mc{2}{c}{\bf\acs{syns}}      & \mc{2}{c}{\bf\acs{dii}}       & \mc{2}{c}{\bf\acl{nyud}}          & \mc{2}{c}{\bf\acs{tum}}       \\  
                                       \cmidrule(lr){3-4}                   \cmidrule(lr){5-6}                   \cmidrule(lr){7-8}              \cmidrule(lr){9-10}             \cmidrule(lr){11-12}            \cmidrule(lr){13-14}            \cmidrule(lr){15-16}            \cmidrule(lr){17-18}                \cmidrule(lr){19-20}  \cmidrule(lr){21-22}
                             & Train &    \acs{rank}\down &        \acs{relimp}\up &        Rel\down &             F\up &         Rel\down &            F\up &      Rel\down &          F\up &      Rel\down &  \acs{d25}\up &      Rel\down &          F\up &      Rel\down &          F\up &      Rel\down &  \acs{d25}\up &       Rel\down &     \acs{d25}\up &      Rel\down &  \acs{d25}\up \\
\midrule
Garg~\cite{Garg2016}         & S     &         7.58 &       -38.52 & \zs\nbest{7.65} & \zs\nbest{53.28} &            27.63 &    \nbest{9.08} &         26.93 &          7.80 &         39.60 &         44.15 &         39.41 & \nbest{31.93} &         26.05 &         15.17 &         19.18 &         70.54 &          22.49 &            59.60 &         23.53 &         62.82 \\ 
Monodepth2~\cite{Godard2019} & MS    &         7.74 &       -38.34 &         \zs7.90 &         \zs50.50 &            27.44 &            7.97 &         24.31 &          8.25 &         39.53 &         44.71 &         40.09 &         29.49 &         25.31 &         14.83 &         19.40 &         70.42 &          22.41 &            60.09 &         23.50 &         62.36 \\ 
DiffNet~\cite{Zhou2021}      & MS    &         7.05 &       -36.84 &         \zs7.98 &         \zs49.60 &            27.46 &            7.76 & \nbest{23.03} &          9.43 & \nbest{38.87} & \nbest{46.14} &         39.93 &         28.77 &         25.09 &         14.64 &         19.11 &         70.94 &          21.82 &    \nbest{61.30} &         23.21 &         63.08 \\ 
HR-Depth~\cite{Lyu2021}      & MS    &         5.95 &       -35.16 &         \zs7.70 &         \zs51.49 &    \nbest{27.01} &            8.39 &         23.13 &  \nbest{9.94} &         39.09 &         45.60 & \nbest{38.82} &         30.90 & \nbest{25.07} & \nbest{15.48} & \nbest{18.93} & \nbest{71.19} &  \nbest{21.74} &            61.18 & \nbest{23.18} & \nbest{63.50} \\ 
\midrule
\textbf{\acs{kbr} (Ours)}    & M     &         3.37 &         0.00 &  \zs\best{6.84} &  \zs\best{56.17} &  \zs\best{14.39} & \zs\best{17.67} &  \best{12.63} & \best{20.21} &  \best{33.49} &      \best{57.08} &  \best{33.34} &  \best{40.81} &  \best{22.40} &  \best{18.50} &  \best{14.91} &      \best{80.77} &  \best{11.59} &      \best{87.23} &  \best{15.02} &      \best{80.86} \\

\midrule
\midrule
MiDaS~\cite{Ranftl2020}      & D     &         4.89 &       -11.84 &           13.71 &            33.44 &            16.96 &           12.62 &         16.00 &         15.41 &         32.72 &         59.04 &         30.95 &         39.55 &         26.94 &         14.69 &        10.71 &         88.42 &           10.48 &            89.59 &         14.43 &         82.35 \\
DPT-ViT~\cite{Ranftl2021}    & D     &         3.32 &        -1.74 &           10.98 &            40.56 &    \nbest{15.52} &           14.46 &         15.49 &         18.25 & \nbest{32.59} & \nbest{59.82} & \nbest{25.53} & \nbest{43.57} & \nbest{23.24} & \nbest{17.44} & \nbest{9.60} & \nbest{91.38} &           10.10 &            90.10 & \nbest{12.68} & \nbest{86.25} \\
DPT-BEiT~\cite{Ranftl2021}   & D     &  \best{1.84} & \best{11.12} & \zs\nbest{9.45} & \zs\nbest{44.22} &     \best{13.55} &    \best{16.58} & \nbest{10.70} & \nbest{22.63} &  \best{31.08} &  \best{61.51} &  \best{21.38} &  \best{46.46} &  \best{21.47} &  \best{17.73} &  \best{7.89} &  \best{93.34} & \zs \best{5.40} & \zs \best{96.54} &  \best{10.45} &  \best{89.68} \\
NeWCRFs~\cite{Weihao2022}    & D     & \nbest{3.26} & \nbest{1.03} &  \zs\best{5.23} &  \zs\best{59.20} &         18.20 & \nbest{15.17} &   \best{9.59} &  \best{23.02} &         37.01 &             49.66 &         39.25 &         32.43 &         24.28 &         16.76 &        14.05 &             84.95 & \zs\nbest{6.22} &     \zs\nbest{95.58} &         14.63 &             82.95 \\
\bottomrule
\end{tabular}

\emph{%
Highlighted cells are \emph{\textbf{NOT zero-shot}} results.
\textbf{S}=Stereo, \textbf{M}=Monocular, \textbf{D}=Ground-truth Depth.
}


==> Tables/supp_motion.tex <==

\scriptsize
\addtolength{\tabcolsep}{0.05em}
\def\mc{\multicolumn}


\mycaption{Monodepth2~\cite{Godard2019} Losses}{%
The minimum reconstruction loss and automasking from Monodepth2 serve as valuable proxies to increase robustness to dynamic objects, while remaining simple and efficient. 
}


\begin{tabular}{@{}lllllllllllllllllllll@{}}
\toprule
                             & \mc{2}{c}{\textbf{Multi-task}} & \mc{2}{c}{\bf\acs{keb}}            & \mc{2}{c}{\bf\acs{mc}}             & \mc{2}{c}{\bf\acs{ddad}}      & \mc{2}{c}{\bf\acs{dio}}       & \mc{2}{c}{\bf\acs{sintel}}    & \mc{2}{c}{\bf\acs{syns}}      & \mc{2}{c}{\bf\acs{dii}}       & \mc{2}{c}{\bf\acl{nyud}}          & \mc{2}{c}{\bf\acs{tum}}       \\  
                                       \cmidrule(lr){2-3}                   \cmidrule(lr){4-5}                   \cmidrule(lr){6-7}              \cmidrule(lr){8-9}             \cmidrule(lr){10-11}            \cmidrule(lr){12-13}            \cmidrule(lr){14-15}            \cmidrule(lr){16-17}                \cmidrule(lr){18-19}  \cmidrule(lr){20-21}
                             &   \acs{rank}\down &        \acs{relimp}\up &        Rel\down &             F\up &         Rel\down &            F\up &      Rel\down &          F\up &      Rel\down &  \acs{d25}\up &      Rel\down &          F\up &      Rel\down &          F\up &      Rel\down &  \acs{d25}\up &       Rel\down &     \acs{d25}\up &      Rel\down &  \acs{d25}\up \\
\midrule
         Baseline & \nbest{1.89} & \nbest{0.00} & \nbest{9.00} & \nbest{53.50} &  \best{16.89} &  \best{14.66} & \nbest{23.57} & \nbest{11.13} & \nbest{35.99} &     \nbest{52.70} & \nbest{35.33} & \nbest{38.15} & \nbest{25.47} & \nbest{15.73} & \nbest{17.91} &     \nbest{75.03} & \nbest{21.68} &     \nbest{71.41} & \nbest{17.69} &     \nbest{75.67} \\ 
MinRec+Automask &  \best{1.11} &  \best{7.01} &  \best{6.50} &  \best{55.62} & \nbest{16.96} & \nbest{14.48} &  \best{18.49} &  \best{11.64} &  \best{35.62} &      \best{52.95} &  \best{34.97} &  \best{38.83} &  \best{24.44} &  \best{16.25} &  \best{16.85} &      \best{76.50} &  \best{14.27} &      \best{80.54} &  \best{17.23} &      \best{76.23} \\ 
\bottomrule
\end{tabular}


==> Tables/supp_res.tex <==
% Supplementary results using median scaling. 

\addtolength{\tabcolsep}{0.2em}
\def\mc{\multicolumn}

\mycaption{Median-Scaling Results}{%
This represents the common \ac{ssmde} evaluation procedure~\cite{Zhou2017}. 
Removing the shift alignment reduces performance for all approaches. 
Our method still outperforms all existing \acl{ssmde} models, and \ac{crf} in many cases.
}


\begin{tabular}{@{}llllllllllllllllllll@{}}
\toprule
                             &       & \mc{4}{c}{\bf In-Distribution}                                         & \mc{8}{c}{\bf Outdoor}                                                                                                        & \mc{6}{c}{\bf Indoor}                                                                            \\
                                       \cmidrule(lr){3-6}                                                       \cmidrule(lr){7-14}                                                                                                             \cmidrule(lr){15-20}
                             &       & \mc{2}{c}{\bf\acs{keb}}            & \mc{2}{c}{\bf\acs{mc}}            & \mc{2}{c}{\bf\acs{ddad}}      & \mc{2}{c}{\bf\acs{dio}}       & \mc{2}{c}{\bf\acs{sintel}}    & \mc{2}{c}{\bf\acs{syns}}      & \mc{2}{c}{\bf\acs{dii}}       & \mc{2}{c}{\bf\acl{nyud}}         & \mc{2}{c}{\bf\acs{tum}}       \\  
                                       \cmidrule(lr){3-4}                   \cmidrule(lr){5-6}                  \cmidrule(lr){7-8}              \cmidrule(lr){9-10}             \cmidrule(lr){11-12}            \cmidrule(lr){13-14}            \cmidrule(lr){15-16}            \cmidrule(lr){17-18}               \cmidrule(lr){19-20}
                             & Train &        Rel\down &             F\up &        Rel\down &            F\up &      Rel\down &          F\up &      Rel\down &  \acs{d25}\up &      Rel\down &          F\up &      Rel\down &          F\up &      Rel\down &  \acs{d25}\up &       Rel\down &    \acs{d25}\up &      Rel\down &  \acs{d25}\up \\
\midrule
Garg~\cite{Garg2016}         & S     & \zs\nbest{7.65} & \zs\nbest{53.28} & \nbest{34.55} & \nbest{9.29} &         26.77 &         4.77 &         57.87 &             42.85 & \nbest{53.16} & \nbest{30.98} &         31.68 &         13.58 &         30.63 &             51.00 &         26.78 &             54.29 & \nbest{27.37} &     \nbest{55.26} \\
Monodepth2~\cite{Godard2019} & MS    &  \zs       7.90 &   \zs      50.50 &         35.88 &         8.18 &         25.46 &         4.77 &         57.61 &             43.21 &         54.40 &         30.11 &         30.05 &         13.28 &         33.51 &             47.49 &         29.87 &             50.08 &         30.59 &             49.82 \\
DiffNet~\cite{Zhou2021}      & MS    &  \zs       7.98 &   \zs      49.60 &         35.50 &         8.15 &         24.17 &         4.75 & \nbest{55.68} &     \nbest{45.37} &         55.23 &         29.44 & \nbest{29.75} &         13.41 & \nbest{28.67} &     \nbest{53.82} & \nbest{26.62} &     \nbest{54.69} &         28.56 &             53.07 \\
HR-Depth~\cite{Lyu2021}      & MS    &  \zs       7.70 &   \zs      51.49 &         35.89 &         8.62 & \nbest{24.01} & \nbest{5.08} &         57.88 &             43.92 &         53.91 &         30.89 &         29.87 & \nbest{14.03} &         32.88 &             47.67 &         27.32 &             53.06 &         29.22 &             52.31 \\
\midrule
\textbf{\acs{kbr} (Ours)}    & M     &  \zs\best{7.23} &  \zs\best{54.63} &  \zs\best{18.73} & \zs\best{15.04} &  \best{14.01} & \best{14.01} &  \best{43.80} &      \best{60.84} &  \best{37.06} &  \best{36.01} &  \best{24.92} &  \best{16.49} &  \best{18.88} &      \best{72.09} &  \best{13.27} &      \best{83.65} &  \best{16.60} &      \best{76.48} \\
\midrule
\midrule
MiDaS~\cite{Ranftl2020}      & D     &         18.45 &         20.13 & \nbest{26.02} &         10.61 &         18.38 &          8.28 &  \best{48.63} &      \best{60.15} &  \best{39.09} &  \best{32.72} &         35.30 &          9.18 & \nbest{18.08} &     \nbest{74.48} & \nbest{23.11} &     \nbest{69.67} & \nbest{17.75} &             76.99 \\ 
DPT-ViT~\cite{Ranftl2021}    & D     & \nbest{14.23} &         36.25 &         28.54 &         11.38 &         17.83 &          8.99 &         72.46 &             49.09 &        128.86 &         29.58 &         32.69 &         12.93 &         36.82 &             55.15 &         24.82 &             67.95 &         24.33 &             78.16 \\ 
DPT-BEiT~\cite{Ranftl2021}   & D     &  \zs       18.20 & \zs\nbest{37.46} &         30.79 & \nbest{12.58} & \nbest{15.39} & \nbest{11.78} &         70.30 &             50.03 &         60.20 &         29.54 & \nbest{31.09} & \nbest{13.76} &         51.07 &             53.11 &    \zs     75.32 &   \zs          42.91 &         25.27 &      \best{83.07} \\ 
NeWCRFs~\cite{Weihao2022}    & D     &  \zs \best{5.55} & \zs \best{56.45} &  \best{22.15} &  \best{13.68} &  \best{11.87} &  \best{13.44} & \nbest{50.52} &     \nbest{51.16} & \nbest{48.42} & \nbest{32.30} &  \best{27.79} &  \best{14.50} &  \best{16.15} &      \best{79.52} &   \zs\best{7.00} &   \zs   \best{94.44} &  \best{14.93} &     \nbest{80.63} \\ 
\bottomrule
\end{tabular}

\emph{%
Highlighted cells are \emph{\textbf{NOT zero-shot}} results.
\textbf{S}=Stereo, \textbf{M}=Monocular, \textbf{D}=Ground-truth Depth.
}

